The JCMT Transient Survey: Six-Year Summary of 450/850\,$\mu$m Protostellar Variability and Calibration Pipeline Version 2.0

The JCMT Transient Survey has been monitoring eight Gould Belt low-mass star-forming regions since December 2015 and six somewhat more distant intermediate-mass star-forming regions since February 2020 with SCUBA-2 on the JCMT at \ShortS and \LongS and with an approximately monthly cadence. We introduce our Pipeline v2 relative calibration procedures for image alignment and flux calibration across epochs, improving on our previous Pipeline v1 by decreasing measurement uncertainties and providing additional robustness. These new techniques work at both \LongS and \ShortNS, where v1 only allowed investigation of the \LongS data. Pipeline v2 achieves better than $0.5^{\prime\prime}$ relative image alignment, less than a tenth of the submillimeter beam widths. The v2 relative flux calibration is found to be 1\% at \LongS and $<5$\% at \ShortNS. The improvement in the calibration is demonstrated by comparing the two pipelines over the first four years of the survey and recovering additional robust variables with v2. Using the full six years of the Gould Belt survey the number of robust variables increases by 50\,\%, and at \ShortS we identify four robust variables, all of which are also robust at \LongNS. The multi-wavelength light curves for these sources are investigated and found to be consistent with the variability being due to dust heating within the envelope in response to accretion luminosity changes from the central source.

==> Referee_Comments.tex <==
Response for the Reviewer

1. The description of the calibration in 4.1 and 4.3 can be confusing - I found myself reading it several times and still not having a completely clear conception of what was done. Here are some suggestions which might help readers:

i. In 4.1, the addition of equations describing the source weighting in steps 1 and 3 would be helpful.

STM: Thank you for pointing this out. I have now rewritten the section describing the weighted calibration procedure, including more equations and splitting the former description into more bite-sized pieces.

ii. Also, a better description of the optimization of the calibrator groups in 4.3 would be helpful. It's a seemingly complicated procedure with a number of trade offs, and it is unclear what choices were ultimately made to resolve the trade offs.

STM: This calibration method is based on the calibration scheme presented in detail in Mairs 2017. The difference here is the way in which we measure peak fluxes (due to the significant alignment improvements), the exclusion of variable sources, and how we select usable 450 micron maps such that we can repeat the method that was originally only applied to 850 micron maps to the shorter, noisier, wavelength. I include more detail on the trade-offs between a higher number of sources and a lower FCF uncertainty in section 4.2 of that paper - and show a plot of the standard deviations of source-pair comparisons there. I have added a statement to this effect, directing readers to the original 2017 calibration paper for more detail. I also added another statement to make more clear that this method is only used as a consistency check to verify the precision of the weighted calibration scheme and it is not used in the production of the co-adds. The main highlight of this verification section is Figure 5/6 which shows consistency between the former method and the more robust method developed in this paper.

iii. Finally, the 2nd half of the discussion of 4.3 - where the discussion transition to the full calibration procedure - might be pushed into its own section. 

STM: The calibrator groups described in 4.3 are used simply as an independent consistency check on the official, weighted  scheme that is used to calibrate the images. Figures 5 and 6, therefore are meant to show that we are highly confident in our final calibration, but these secondary calibrator "families" are not actually used to produce the co-adds. For this reason, I kept this discussion in a subsection, but I agree a new Section was needed that distinguished the final co-adds from the calibration discussion, above. I have therefore moved the co-add discussion into its own section. 

2. In either the primary or secondary calibration, can the calibration be improved by avoiding protostars, i.e. cores with known IR sources? A brief description of how many of the sources/how much of the source flux used in the calibration are from starless gas vs protostars cores might be useful.

STM: Thanks for this great point -- with the restructuring of the description, above, I have highlighted that known variables are used in both the calibration and the consistency-check calibration, but only protostars themselves, which do not show variability, are still included. We performed testing and the calibration does not improve if we leave out all protostars - in fact, we then have less bright/reliable sources with which we can perform the calibration, which increases the uncertainty. If a protostar previously used in the calibration begins to exhibit variability, the weighted algorithm automatically down-weights that source's contribution and we can manually remove the variable source. The other calibration method is only used as a consistency check, but a newly-varying protostar will yield a deviation from the norm when comparing the two methods and the source is identifiable in that algorithm as well. I added text after the description of the weighted algorithm to highlight that the method of retaining all known non-varying protostars in the pool of calibrators can be used over time to identify newly varying YSOs and previously undiscovered YSOs such as deeply embedded protostars that were historically too faint to be included
in previous surveys. Therefore, the fraction of sources that are starless (or, deemed starless depending on survey thresholds) does not affect the overall calibration - only the source brightness and the consistency of the signal over time affect the results.


3. In tables 4 and 5, it is not clear to me what a period means for a linear, or even curved light curve. In particular, without any sort of uncertainty, the inclusion of periods for every source seems misleading.

STM: Thanks for highlighting the need for some additional text, here. We are following the same methods used in Lee et al. 2021 for consistency with previous literature using the JCMT transient data. Here, we use a longer timescale and both SCUBA-2 wavelengths (Lee et al. focused on 850 microns only). Using these methods for a consistent comparison, every lightcurve has a best-fit sinusoid, regardless if it is a periodic, curved, linear, or even a non-variable source. The FAP value for non-variable sources, for example, will be high too high to consider the fit physically meaningful. Furthermore, as these period fits assume an underlying sinusoid the derived values should be taken as representative of the quantitative nature, rather than specific. For timescales shorter than the observing window the periods reasonable measure of episodic timescale whereas for longer derived periods the uncertainties are necessarily much larger. Given the <10-year timescales of these observations, there is insufficient data to distinguish linearly varying sources from sources with sinusoidal variability over long periods, since sinusoids can be regarded as a straight line near its zeros when the period is long. Variables with periods longer than 20 years are, therefore, classified as 'linear', but also assigned a derived period. Further observations over the coming years may refine these fits and allow for differentiation in the future. 

We have included additional explanation in Section 6/6.1.

The uncertainty of these fits is explored by comparing our historic/new calibration methods and our 4-year to 6-year observing windows (Figure 9), though the manner and timescales over which these lightcurves evolve is still an active area of study and current long period predictions must be tested as more data are collected (Figure 12/HOPS 358 is a great example of this since a linear variable became obviously sinusoidal with only 2 additional years of observations due to a dramatic turn-around in flux). The False Alarm Probability is the value used to validate the detection/goodness of fit/classification, but it can not be used to derive physically meaningful uncertainties on the period value, even using bootstrapping methods. 

4. It's worth noting that the J182947.6+011553 source is not in Spitzer 24 or 4.5 micron data, nor is it in the eHOPS catalog in IRSA. Could this source be a background galaxy? 

STM: Text updated to include this point  - thank you!

5. Picky comment: the text says "fields contain more than 300Class 0/I/Flat young stellar objects (YSOs) and more than 1400 Class II sources". YSOs is usually applied as an umbrella term to include all Class 0/I/Flat Spectrum protostars and Class II objects, and to minimize confusion in nomenclature it would be good to keep to this usage.

STM: Updated! Thank you very much.


We have also included an acknowledgement that these comments have significantly strengthened this work - thank you! 
